BalanceVR: Balance Training to Increase Tolerance to Cybersickness in Immersive Virtual Reality

Cybersickness is a serious usability problem in virtual reality. Postural (or balance) instability theory has emerged as one of the major hypotheses for the cause of cybersickness. In this paper, we conducted a two-week-long experiment to observe the trends in user balance learning and sickness tolerance under different experimental conditions to analyze the potential inter-relationship between them. The experimental results have shown, aside from the obvious improvement in balance performance itself, that accompanying balance training had a stronger effect of increasing tolerance to cybersickness than mere exposure to VR. In addition, training in immersive VR was found to be more effective than using the 2D-based non-immersive medium, especially for the transfer effect to other non-training VR content.

==> sections/00_abstract.tex <==
%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}
Cybersickness is a serious usability problem in virtual reality.  
Postural (or balance) instability theory has emerged as one of the major hypotheses for the cause of cybersickness.  
In this paper, we conducted a two-week-long experiment to observe the trends in user balance learning and sickness tolerance under different experimental conditions to analyze the potential inter-relationship between them.  
The experimental results have shown, aside from the obvious improvement in balance performance itself, that accompanying balance training had a stronger effect of increasing tolerance to cybersickness than mere exposure to VR.  
In addition, training in immersive VR was found to be more effective than using the 2D-based non-immersive medium, especially for the transfer effect to other non-training VR content.
\end{abstract}
